Unselfie: Translating Selfies to Neutral-pose Portraits in the Wild

Due to the ubiquity of smartphones, it is popular to take photos of one's self, or "selfies." Such photos are convenient to take, because they do not require specialized equipment or a third-party photographer. However, in selfies, constraints such as human arm length often make the body pose look unnatural. To address this issue, we introduce $\textit{unselfie}$, a novel photographic transformation that automatically translates a selfie into a neutral-pose portrait. To achieve this, we first collect an unpaired dataset, and introduce a way to synthesize paired training data for self-supervised learning. Then, to $\textit{unselfie}$ a photo, we propose a new three-stage pipeline, where we first find a target neutral pose, inpaint the body texture, and finally refine and composite the person on the background. To obtain a suitable target neutral pose, we propose a novel nearest pose search module that makes the reposing task easier and enables the generation of multiple neutral-pose results among which users can choose the best one they like. Qualitative and quantitative evaluations show the superiority of our pipeline over alternatives.

==> supp_Fig_inpaintBG.tex <==


\begin{figure}
\centering
% \captionsetup{justification=centering}
\captionsetup{font=small,labelfont=normalsize,justification=centering}

\begin{subfigure}[b]{.19\linewidth}
\caption*{Input selfie}
\vspace{-1mm}
\begin{overpic}[width=\linewidth]{figures/supp_inpaintBG/206713499_InputSelfie.png}
\put(0,665) {\scalebox{0.65}{\id{206713499}}}
\end{overpic}
% \includegraphics[width=\linewidth]{figures/supp_inpaintBG/206713499_InputSelfie.png}
\end{subfigure}
%
\begin{subfigure}[b]{.19\linewidth}
% \caption*{Input BG $I_{bg}$}
\caption*{BG $I_{bg}$}
\vspace{-1mm}
\includegraphics[width=\linewidth]{figures/supp_inpaintBG/206713499_BG.png}
\end{subfigure}
%
\begin{subfigure}[b]{.19\linewidth}
% \caption*{Input inpainted BG $I_{bg}$}
\caption*{Inpainted BG $I_{ibg}$}
\vspace{0mm}
\includegraphics[width=\linewidth]{figures/supp_inpaintBG/206713499_inpaintBG.png}
\end{subfigure}
%
\begin{subfigure}[b]{.19\linewidth}
% \caption*{Result}
\caption*{Result with $I_{bg}$}
\vspace{-1mm}
\includegraphics[width=\linewidth]{figures/supp_inpaintBG/206713499_Ours.png}
\end{subfigure}
%
\begin{subfigure}[b]{.19\linewidth}
% \caption*{Result \\(inpainted BG)}
\caption*{Result with $I_{ibg}$}
\vspace{0mm}
\includegraphics[width=\linewidth]{figures/supp_inpaintBG/206713499_Ours_inpaintBG.png}
\end{subfigure}


\begin{subfigure}[b]{.19\linewidth}
% \caption*{Input selfie}
\vspace{-1mm}
\begin{overpic}[width=\linewidth]{figures/supp_inpaintBG/138378456_InputSelfie.png}
\put(0,665) {\scalebox{0.65}{\id{138378456}}}
\end{overpic}
% \includegraphics[width=\linewidth]{figures/supp_inpaintBG/138378456_InputSelfie.png}
\end{subfigure}
%
\begin{subfigure}[b]{.19\linewidth}
% \caption*{Ours}
\vspace{-1mm}
\includegraphics[width=\linewidth]{figures/supp_inpaintBG/138378456_BG.png}
\end{subfigure}
%
\begin{subfigure}[b]{.19\linewidth}
% \caption*{Ours \\(inpainted background)}
\vspace{0mm}
\includegraphics[width=\linewidth]{figures/supp_inpaintBG/138378456_inpaintBG.png}
\end{subfigure}
%
\begin{subfigure}[b]{.19\linewidth}
% \caption*{Ours}
\vspace{-1mm}
\includegraphics[width=\linewidth]{figures/supp_inpaintBG/138378456_Ours.png}
\end{subfigure}
%
\begin{subfigure}[b]{.19\linewidth}
% \caption*{Ours \\(inpainted background)}
\vspace{0mm}
\includegraphics[width=\linewidth]{figures/supp_inpaintBG/138378456_Ours_inpaintBG.png}
\end{subfigure}


\begin{subfigure}[b]{.19\linewidth}
% \caption*{Input selfie}
\vspace{-1mm}
\begin{overpic}[width=\linewidth]{figures/supp_inpaintBG/225137362_InputSelfie.png}
\put(0,665) {\scalebox{0.65}{\id{225137362}}}
\end{overpic}
% \includegraphics[width=\linewidth]{figures/supp_inpaintBG/225137362_InputSelfie.png}
\end{subfigure}
%
\begin{subfigure}[b]{.19\linewidth}
% \caption*{Ours}
\vspace{-1mm}
\includegraphics[width=\linewidth]{figures/supp_inpaintBG/225137362_BG.png}
\end{subfigure}
%
\begin{subfigure}[b]{.19\linewidth}
% \caption*{Ours \\(inpainted background)}
\vspace{0mm}
\includegraphics[width=\linewidth]{figures/supp_inpaintBG/225137362_inpaintBG.png}
\end{subfigure}
%
\begin{subfigure}[b]{.19\linewidth}
% \caption*{Ours}
\vspace{-1mm}
\includegraphics[width=\linewidth]{figures/supp_inpaintBG/225137362_Ours.png}
\end{subfigure}
%
\begin{subfigure}[b]{.19\linewidth}
% \caption*{Ours \\(inpainted background)}
\vspace{0mm}
\includegraphics[width=\linewidth]{figures/supp_inpaintBG/225137362_Ours_inpaintBG.png}
\end{subfigure}


\caption{Results of using inpaited background.}
\label{supp_fig:inpaintBG}
\end{figure}
